Continuous Optimization for Satisfiability Modulo Theories on Linear Real Arithmetic

Efficient solutions for satisfiability modulo theories (SMT) are integral in industrial applications such as hardware verification and design automation. Existing approaches are predominantly based on conflict-driven clause learning, which is structurally difficult to parallelize and therefore scales poorly. In this work, we introduce FourierSMT as a scalable and highly parallelizable continuous-variable optimization framework for SMT. We generalize the Walsh-Fourier expansion (WFE), called extended WFE (xWFE), from the Boolean domain to a mixed Boolean-real domain, which allows the use of gradient methods for SMT. This addresses the challenge of finding satisfying variable assignments to high-arity constraints by local updates of discrete variables. To reduce the evaluation complexity of xWFE, we present the extended binary decision diagram (xBDD) and map the constraints from xWFE to xBDDs. We then show that sampling the circuit-output probability (COP) of xBDDs under randomized rounding is equivalent to the expectation value of the xWFEs. This allows for efficient computation of the constraints. We show that the reduced problem is guaranteed to converge and preserves satisfiability, ensuring the soundness of the solutions. The framework is benchmarked for large-scale scheduling and placement problems with up to 10,000 variables and 700,000 constraints, achieving 8-fold speedups compared to state-of-the-art SMT solvers. These results pave the way for GPU-based optimization of SMTs with continuous systems.

==> notes/MP-proof.tex <==
To prove Theorem~\ref{thm:forward}, we first reproduce Lemma 2 in~\cite{kyrillidis2021continuous}. 
\begin{lemma}\label{lmm:forward}
    Let $G_c(V_c, E_c)$ be an XBDD encoded constraint $c$ and run Algorithm~\ref{alg:forward} on $G_c$. 
    For a real assignment $(a, b)\in[-1,1]^n\times\mathbb{R}^m$, we have
    \begin{align*}
        \mathbb{P}[x_i=-1] &= \frac{1-a_i}{2}, \\
        \mathbb{P}[\delta_i(b)=-1] &= \frac{1-d_i(b)}{2}.
    \end{align*}
    Then for each node $v\in{}V_c$, we have
    \begin{equation*}
        m_{td}[v] = {Pr}(G_c,v),
    \end{equation*}
    where ${Pr}(G_c,v)$ is the probability that the node $v$ is on the path generated by $x$ and $d(\cdot)$ on $G_c$.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lmm:forward}]
    We prove the statement by structural induction on XBDD $G_c$.
    We first denote 
    \begin{equation*}
        z = \left[\begin{array}{cccccc}
             \mathbb{P}[x_1=-1] & ... & \mathbb{P}[x_n=-1] &
            \mathbb{P}[d_1(b)=-1] & ... & \mathbb{P}[d_k(b)=-1]
        \end{array}\right]
    \end{equation*}
    
    \noindent\textbf{Basic step}: For the root node $r$ of $G_c$, 
    \begin{equation*}
        m_{td}[v] = 1, 
    \end{equation*}
    where the statement holds because $r$ is on the path generated by every discrete assignment on $G_c$. \\
    
    \noindent\textbf{Inductive step}: For each non-root node $v$ of $G_c$, let ${par}_T(v)$ be the set of parents of $v$ with an edge labeled by \textsc{True} and ${par}_F(v)$ be the set of parents of $v$ with an edge labeled by \textsc{False} in XBDD $G_c$. 
    After algorithm~\ref{alg:forward} terminates, we have
    \begin{equation*}
        m_{td}[v] = \sum_{u\in{par}_T(v)} z_i \cdot m_{td}[u] + \sum_{u\in{par}_T(v)} (1-z_i) \cdot m_{td}[u] 
    \end{equation*}
    By inductive hypothesis, 
    \begin{align*}
        m_{td}[v] 
        &= \sum_{u\in{par}_T(v)}  z_i \cdot{Pr}(G_c,u) + \sum_{u\in{par}_T(v)}  (1-z_i) \cdot{Pr}(G_c,u) \\
        &=  {Pr}(G_c,v) 
    \end{align*}
    The last inequality holds because the events of reaching $v$ from different parents are exclusive.
\end{proof}

The above Lemma shows that, after running Algorithm~\ref{alg:forward}, we have
\begin{align*}
    m_{td}[V_c[T]] &= {Pr}(G_c,V_c[T]) \\
    & = {COP}_c(\mathcal{P}_\sigma) \text{\qquad(By definition of circuit-output probability)}
\end{align*}

\noindent\textbf{Complexity}: 
Algorithm~\ref{alg:forward} traverse all XBDD $G_c$ for all $c\in{}C$. 
The topological sort takes $O(|V_c|+|E_c|)$ time by Kahn's algorithm. 
The message propagation takes $O(|E_c|)$ time. 
Since $|E_c|=2|V_c|$, \emph{i.e.}, all non-terminal nodes in XBDD only have two outgoing edges. 
Hence, the overall complexity scales at $O(|V_c|)$.

To prove Theorem~\ref{thm:backward}, we first reproduce Lemma 4 in~\cite{kyrillidis2021continuous}. 
\begin{lemma}\label{lmm:backward}
    Let $G_c(V_c, E_c)$ be an XBDD encoded constraint $c$ and run Algorithm~\ref{alg:backward} on $G_c$. 
    For a real assignment $(a, b)\in[-1,1]^n\times\mathbb{R}^m$, we have
    \begin{align*}
        \mathbb{P}[x_i=-1] &= \frac{1-a_i}{2}, \\
        \mathbb{P}[\delta_i(b)=-1] &= \frac{1-d_i(b)}{2}.
    \end{align*}
    Then, for each node $v\in{}V_c$, let $f_{c,v}$ be the subfunction corresponding to the sub-XBDD generated by regarding $v$ as the root. 
    The following holds:
    \begin{equation*}
        m_{bu}[v] = {COP}_{c,v}(P_\sigma).
    \end{equation*}
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lmm:backward}]
    We prove the statement by structural induction on XBDD $G_c$.
    We first denote 
    \begin{equation*}
        z = \left[\begin{array}{cccccc}
             \mathbb{P}[x_1=-1] & ... & \mathbb{P}[x_n=-1] &
            \mathbb{P}[d_1(b)=-1] & ... & \mathbb{P}[d_k(b)=-1]
        \end{array}\right]
    \end{equation*}
    
    \noindent\textbf{Basic step}: For the terminal nodes, we have
    \begin{align*}
        m_{bu}[V_c[T]] &= 1,\\
        m_{bu}[V_c[F]] &= 0.
    \end{align*}
    Since the subfunctions given by \textsc{True} and \textsc{True} are just Boolean constants, the statement holds. 
    
    \noindent\textbf{Inductive step}: For each non-terminal node $v$ of $G_c$, after algorithm~\ref{alg:backward} terminates, we have
    \begin{equation*}
        m_{bu}[v] = \frac{1-z_i}{2} \cdot m_{bu}[v.T] + \frac{1+z_i}{2} \cdot m_{bu}[v.F]
    \end{equation*}
    By inductive hypothesis, 
    \begin{align*}
        m_{bu}[v] 
        &= \frac{1-z_i}{2} \cdot COP_{c,v.T}(P_\sigma)+ \frac{1+z_i}{2} \cdot COP_{c,v.F}(P_\sigma) \\
        &= COP_{c,v}(P_\sigma)
    \end{align*}
\end{proof}

With Lemma~\ref{lmm:forward} and Lemma~\ref{lmm:backward}, we are ready to prove Theorem~\ref{thm:backward}.
Given an XBDD $G_c$, we expand all terminal nodes such that each can have only one parent node. 
The expanded XBDD is called $G_{c'}$, which has a true terminal set $T$ and a false terminal set $F$. 
By repeating the proof of Lemma~\ref{lmm:forward} and Lemma~\ref{lmm:backward} on $G_{c'}$, for any non-terminal node $v\notin(T\cup F)$, we have
\begin{align*}
    m_{td}'[v] &= m_{td}[v] \\
    m_{bu}'[v] &= m_{bu}[v]
\end{align*}
For any true terminal node $v\in{}T$ and false terminal node $u\in{}F$, we have
\begin{align*}
    m_{bu}'[v] &= 1 \\
    m_{bu}'[u] &= 0
\end{align*}

\begin{align*}
    COP_c(\mathcal{P}_\sigma) 
    &=\mathbb{P}[f_c=-1|\mathcal{P}_\sigma]\\
    &= \sum_{v\in \{u:id(u)=i\}}{Pr}(G_c', v) \cdot \mathbb{P}[f_c=-1|v, \mathcal{P}_\sigma] \\
    &= \sum_{v\in \{u:id(u)=i\}}m_{td}'[v] \cdot m_{bu}'[v] \\
    &= \sum_{v\in \{u:id(u)=i\}}m_{td}[v] \cdot m_{bu}[v] \\
    &= \sum_{v\in \{u:id(u)=i\}}m_{td}[v] \cdot \left(z_i\cdot m_{bu}[v.T] + (1-z_i)\cdot m_{bu}[v.F]\right)
\end{align*}

Hence we have

\begin{align*}
    \frac{\partial COP_c(\mathcal{P}_\sigma)}{\partial z_i}
    &= \sum_{v\in \{u:id(u)=i\}}m_{td}[v] \cdot \left( m_{bu}[v.T] - m_{bu}[v.F]\right) \\
    \frac{\partial f_c(a, b)}{\partial z_i}
    &= \sum_{v\in \{u:id(u)=i\}}m_{td}[v] \cdot \left( m_{bu}[v.F] - m_{bu}[v.T]\right)
\end{align*}

\noindent\textbf{Complexity}: 
Algorithm~\ref{alg:forward} traverse all XBDD $G_c$ for all $c\in{}C$. 
The topological sort takes $O(|V_c|+|E_c|)$ time by Kahn's algorithm. 
The message propagation takes $O(|E_c|)$ time. 
For gradient computation, the worst case is that every literal is an atomic constraint that consists of all $m$ real variables. 
Therefore, the gradient computation takes $O(m\cdot|E_c|)$ time. 
Since $|E_c|=2|V_c|$, \emph{i.e.}, all non-terminal nodes in XBDD only have two outgoing edges. 
Hence, the overall complexity scales at $O(m\cdot|V_c|)$.

==> notes/benchmarks.tex <==

\noindent\textbf{Scheduling Benchmarks}. 
The scheduling benchmarks are inspired by classical job–machine assignment problems, a central domain in operations research. 
Each instance is parameterized by the number of workers $n_w\in\{16,32,64,128,256\}$ and the job-to-worker ratio $r\in\{2,3,4,5\}$, which together determine the number of jobs as $n_j = r\cdot n_w$. 

The problem is encoded using the following variables:
\begin{itemize}
    \item Worker index: for each job $j$, we use a variable $X_{id,j}\in\{0,...,n_w-1\}$ to encode which worker it is assigned to.
    $X_{id,j}$ is Booleanized as follows
    \begin{equation*}
        X_{id,j} = \sum_{i=0}^{\log_2(n_w)-1}2^i \cdot [x_{i,j}=True].
    \end{equation*}
    For example, with $n_w=16$, indices range from 0 to 15; if
    \begin{equation*}
        \left[\begin{array}{cccc}
            x_{0,0} &  x_{1,0} & x_{2,0} & x_{3,0} 
        \end{array}\right] = 
        \left[\begin{array}{cccc}
            True &  True & True & True 
        \end{array}\right],
    \end{equation*}
    then job 0 is assigned to worker 15.
    \item Job start time: job $j$ is launched at $y_j\in\mathbb{R}$.
\end{itemize}

For each $(n_w, r)$ category, we generated 10 random instances by varying:
\begin{itemize}
    \item Worker start time: worker will start admitting job after $d_{id}\in\mathbb{R}$ time, which is sampled from $\mathcal{U}(0,1)$. 
    \item Job run time: to complete job $j$ need $t_j\in\mathbb{R}$ time, which is sampled from $\mathcal{U}(0,1)$. 
    \item Cutoff time: all workers will stop after $d_{id}+T$ time, where $T$ is a solution from a greedy heuristic to ensure feasibility.
\end{itemize}

The problems include the following constraints
\begin{itemize}
    \item Task dependency: if the input of a job $j$ depends on the output of another job $j'$, then $j$ has to be executed after $j'$. 
    \begin{equation*}
        y_j \geq y_{j'} + t_{j'}
    \end{equation*}
    \item Non-overlap: one worker can run only one at a time. 
    Hence, for every pair of jobs $(j, j')$, we need to satisfy
    \begin{equation*}
        \left(\bigvee_{i=0}^{\log_2(n_w)-1}\left(x_{i,j}\oplus{}x_{i,j'}\right)\right) \vee (y_j - y_{j'} \geq t_{j'}) \vee (y_{j'} - y_j \geq t_j).
    \end{equation*}
    \item Feasibility: the job can only run on a worker if the worker is active. 
    Hence, for each job $j$, we need to satisfies
    \begin{equation*}
        \left(\bigvee_{i=0}^{\log_2(n_w)-1}\neg x_{i,j}\right) \vee (y_j \geq d_{id}) \vee (y_j \leq d_{id} + T - t_j).
    \end{equation*}
\end{itemize}

\noindent\textbf{Placement Benchmarks}.
The placement benchmarks model three-dimensional very-large-scale integration (3D VLSI) design, where macros and functional units must be positioned across multiple layers subject to geometric and routing-aware constraints.  

Each instance is parameterized by the number of macros $n_m \in \{2,4,8,16,32,64\}$ and the number of layers $n_\ell \in \{2,4,8\}$. For each $(n_m,n_\ell)$ configuration, we generate 10 random instances, yielding 180 in total.  


\emph{Encoding.} Placement is represented by Booleanized indices and real-valued coordinates:  
\begin{itemize}
    \item Macro index: for each module $j$, a variable $M_{id,j} \in \{0,\dots,n_m-1\}$ encodes the macro assignment, Booleanized as    
    \begin{equation*}
        M_{id,j} = \sum_{i=0}^{\log_2(n_m)-1}2^i \cdot [m_{i,j}=True].
    \end{equation*}
    \item Layer index: a variable $L_{id,j} \in \{0,\dots,n_\ell-1\}$ encodes the assigned layer, Booleanized as
    \begin{equation*}
        L_{id,j} = \sum_{i=0}^{\log_2(n_l)-1}2^i \cdot [l_{i,j}=True].
    \end{equation*}
    \item Coordinates: each module $j$ has continuous position variables $(x_j,y_j) \in \mathbb{R}^2$.  
\end{itemize}

For each $(n_w, r)$ category, we generated 10 instances.
Each instance contains:  
\begin{itemize}
    \item $n_m$ macros, each occupying $1 \times 1$ nm.  
    \item $n_m$ large process elements ($0.4 \times 0.4$ nm) and $n_m \cdot n_\ell$ small process elements ($0.2 \times 0.2$ nm).  
    \item $n_m$ large memory elements ($0.1 \times 0.1$ nm) and $\tfrac{n_m \cdot n_\ell}{2}$ small memory elements ($0.1 \times 0.05$ nm).  
\end{itemize}  

Randomization is applied by alternating the alignment of small memory elements along the $x$- or $y$-axis.
The dimensions of each module are denoted by $w_j$ (width along $x$) and $d_j$ (height along $y$).

The problems include the following constraints
Three classes of constraints are enforced:  
\begin{itemize}
    \item \emph{Routing-aware:} each large process is paired with a large memory, and each small process with two small memories. For associated modules $(j,j')$,  
    \begin{equation*}
        \bigwedge_{i=0}^{\log_2(n_m)-1}\left(m_{i,j}=m_{i,j'}\right) \wedge (x_j - x_{j'} \le w_{j'}) \wedge (x_{j'} - x_j \le w_j) \wedge (y_j - y_{j'} \le h_{j'}) \wedge (y_{j'} - y_j \le h_j)
    \end{equation*}
    \emph{i.e.}, they should be placed in the same macro and should be adjacent to each other. 
    Such that the length of the metal wire can be reduced in the preceding routing stage. 
    \item Non-overlap: modules sharing the same macro and layer must not overlap. For pairs $(j,j')$:  
    \begin{equation*}
        \left(\bigvee_{i=0}^{\log_2(n_m)-1}\left(m_{i,j}\oplus{}m_{i,j'}\right)\right) \vee \left(\bigvee_{i=0}^{\log_2(n_l)-1}\left(l_{i,j}\oplus{}l_{i,j'}\right)\right)
        \vee (x_j - x_{j'} \ge w_{j'}) \vee (x_{j'} - x_j \ge w_j) \vee (y_j - y_{j'} \ge h_{j'}) \vee (y_{j'} - y_j \ge h_j)
    \end{equation*}
    \item Feasibility: all modules must remain within the macro boundary, 
    \begin{equation*}
        (x_j \ge 0) \wedge (x_j \le 1 - w_j) \wedge (y_j \ge 0) \wedge (y_j \le 1 - d_j)
    \end{equation*}
\end{itemize}

\noindent\textbf{Summary}. 
This construction yields 200 plus 180 instances in total, systematically spanning from small to large scales. 
The benchmarks are designed so that small cases are trivially satisfiable, while larger cases create highly constrained, industrial-scale SMT(LRA) problems that stress solver scalability.

==> notes/continuous.tex <==
\subsection{Continuous Optimization} 

\textcolor{red}{[I feel this section can be removed, for a couple of reasons. We do already the relaxation in the section before -- if that section can be expanded / restructured, then we can mention in one paragraph that we need corrections and project back (first paragraph here). Afterwards -- the example  can be hinted at at the end of the paragraph, mentioning that fig 2 illustrates that point for a concrete example. The smoothness properties / the lipschitz constants, the theorems after... everthing goes in the supplementary and we just add one single sentence saying that we discuss this in greater detail in supplementary note xx. In case there is important stuff included in the supplemental (e.g. a general convergence theorem or something) we could just add a sentence saying that we showed in supplemental xy that such gradient projection methods will converge to...]}


Eq.~\eqref{eq:expectation2} is defined on $[-1,1]^n \times \mathbb{R}^m$, meaning that a gradient update may move the Boolean relaxation variables $a$ outside $[-1,1]^n$.  
Such points lie outside the probabilistic interpretation of the relaxation and therefore require correction.  
This motivates the use of projected gradient methods: after each update, if the new point falls outside the feasible domain, it is projected back (see Method section).  

We illustrate a representative example in Fig.~\ref{fig:bdd} to examine the empirical behavior of the projected gradient method.
In particular, we study how the smoothness properties derived in Propositions~\ref{prop:lipschitz}–\ref{prop:nesterov} (see Supplementary Note~\ref{note:smoothness}) affect practical convergence with Lipschitz constants
\begin{align*}
    L_\mathcal{C} &=\alpha\sqrt{n+m}\max\left(1,\frac{\beta}{\sqrt{2\pi}\sigma}\right), \\
    L_{\nabla\mathcal{C}} &=\left(n+\frac{\beta m}{\sqrt{2\pi}\sigma}\right)^\frac{1}{2}L_\mathcal{C}.
\end{align*}
Particularly, we showed by Theorem~\ref{thm:max_step} in Supplementary Note~\ref{note:smoothness} that, with step size $\eta=\frac{1}{L_{\nabla\mathcal{C}}}$, the projected gradient descent converges to an $\epsilon$-projected-critical point in $\mathcal{O}(\frac{\alpha L_{\nabla\mathcal{C}}}{\epsilon^2})$ iterations.

For different sampling radius $\sigma$, the maximum number of gradient steps required to reach a local optimum varies, with the theoretical bound given above:
\begin{align*}
    ub(\sigma) &= 2000\sqrt{3}\left(2+\frac{1}{\sqrt{2\pi}\sigma}\right)^\frac{1}{2}\max\left(1,\frac{1}{\sqrt{2\pi}\sigma}\right)
\end{align*}
In Fig.~\ref{fig:bdd}b-i, the initial point $y_0$ is chosen as
\begin{equation*}
    y_0=-\left(-2\sigma^2\ln\sqrt{2\pi}\sigma\right)^\frac{1}{2}\Big|_{\sigma=0.1},
\end{equation*}
so that all trials cross the transition region and converge to $y > 0$.
The observed number of iterations until convergence aligns closely with the bound $ub(\sigma)$.
In Fig.~\ref{fig:bdd}b-ii, the initial point is instead placed farther from the decision boundary, i.e.,
\begin{equation*}
    y_0=-\max_{\sigma\in[0.1,10]}\left(-2\sigma^2\ln\sqrt{2\pi}\sigma\right)^\frac{1}{2},
\end{equation*}
in which case runs with $\frac{1}{\sigma} \geq 0.74$ fail to cross the transition region and instead converge to $y < 0$.
